Stabilization and Optimal Control of Interconnected SDE - Scalar PDE System

In this paper, we design a controller for an interconnected system consisting of a linear Stochastic Differential Equation (SDE) actuated through a linear hyperbolic Partial Differential Equation (PDE). Our approach aims to minimize the variance of the state of the SDE component. We leverage a backstepping technique to transform the original PDE into an uncoupled stochastic PDE. As such, we reformulate our initial problem as the control of a delayed SDE with a non-deterministic drift. Under standard controllability assumptions, we design a controller steering the mean of the states to zero while keeping its covariance bounded. As final step, we address the optimal control of the delayed SDE employing Artstein's transformation and Linear Quadratic stochastic control techniques.

==> texte_non_utilise.tex <==











Our goal is to find the appropriate functions so that $\alpha$ and $\beta$ verify the following target system
\begin{equation}\label{eq:first_target_system}
\left\{
\begin{array}{l}
     dX(t) = ( (A - BK) X(t) + B \beta(t,0) ) dt + \sigma(t) dW_t \\
     d\alpha(t,x) + \lambda \alpha_x(t,x) dt = \gamma_\alpha(x) \sigma(t) dW_t \\
     d\beta(t,x) - \mu \beta_x(t,x) dt = \gamma_\beta(x) \sigma(t) dW_t \\
     \alpha(t,0) = Q \beta(t,0) \\
     \beta(t,1) = V_{in}(t) +  \\
     X(0) = X_0, \quad \alpha(0,x) = \alpha_0(x), \quad \beta(0,x) = \beta_0(x),
\end{array} 
\right.
\end{equation}
where $V_{eff}$ is the effective control input in the target system, and $K$ is a matrix of our choosing. We show later that the control $V_{in}$ associated to a desired effective control $V_{eff}$ is well posed and can be explicitly determined from the solutions of the system. \textcolor{blue}{We can use the backstepping transformation to add a term $-B K X(t)$ into the SDE. This is done by changing the initial condition on $\gamma_\beta$ to $\gamma_\beta(0) = K$. This is often used in the deterministic case to provide a predictor that stabilizes the dynamic. At first glance, it seems as it could reduce the uncertainty in the system by providing a non delayed feedback. However the initial condition on $\gamma_\beta$ is propagated in the term $\gamma_\beta(x) \sigma(t) dW_t$ and adds an extra uncertainty term in $\beta(t,0)$, which is exactly equal to the uncertainty lost. }


\textcolor{red}{We define the control law $V_BS$ such that ... , Mind that supprressing the term $R u(t,1)$ causes ... (operator not stricly proper)}
\textcolor{orange}{Commentaire important : compared to the classical litterature papier Jean Florent,  we obtain some addtional terms due to the additive noise in the SDE that goes back to the PDE through the coupling. Without the noise, the system would be exponentially stable}




\textcolor{blue}{The following part is there for completeness but will probably be cut out in the final version. We will directly give the kernel equations.} Let us now determine the \textit{kernel equations}, that is the equations that the kernels and the functions $\gamma$ need to verify in order to be solutions of the target system \eqref{eq:first_target_system}. By differentiating $\alpha$ with respect to time in \eqref{eq:backstepping_transform_alpha_beta_definition} we get
\begin{equation*}
\begin{split}
d\alpha(t,x) & = \left[ u_t(t,x) + \int_0^x K_{uu}(x,y) u_t(t,y) dy \right. \\ 
& + \left. \int_0^x K_{uv}(x,y) v_t(t,y) dy \right]dt + \gamma_\alpha(x) dX(t)  \\
& = \left[ - \lambda u_x(t,x) + \eta^{+-}(x) v(t,x) \right] dt \\
& \left[ - \int_0^x K_{uu}(x,y) \lambda u_x(t,y) dy \right. \\
& \quad \left. + \int_0^x K_{uu}(x,y) \eta^{+-}(y) v(t,y) dy \right. \\
& \left. + \int_0^x K_{uv}(x,y) \mu v_x(t,y) dy \right. \\
& \quad \left.+ \int_0^x K_{uu}(x,y) \eta^{-+}(y) u(t,y) dy \right] dt\\
& + \gamma_\alpha(x) ( A X(t) + Bv(t,0) ) dt  + \gamma_\alpha(x) \sigma(t) dW_t
\end{split}
\end{equation*}
by doing a integration by part, we finally get
\begin{equation*}
\begin{split}
d\alpha(t,x) & = \left[ - \lambda u_x(t,x) + \eta^{+-}(x) v(t,x) \right] dt \\
& + \left[ - K_{uu}(x,x) \lambda u(t,x) + K_{uu}(x,0) \lambda u(t,0) \right. \\ 
& \hspace{3em} \left. + \int_0^x (K_{uu})_y(x,y) \lambda u(t,y) dy \right] dt \\
& + \left[  K_{uv}(x,x) \mu v(t,x) - K_{uv}(x,0) \mu v(t,0) \right. \\
& \hspace{3em} \left. - \int_0^x (K_{uv})_y(x,y) \mu v(t,y) dy \right] dt \\
& + \left[ \int_0^x K_{uu}(x,y) \eta^{+-}(y) v(t,y) dy \right. \\
& \quad  \left. + \int_0^x K_{uv}(x,y) \eta^{-+}(y) u(t,y) dy \right] dt\\
& + \gamma_\alpha(x) ( A X(t) + Bv(t,0) ) dt  + \gamma_\alpha(x) \sigma(t) dW_t
\end{split}
\end{equation*}
On the other hand, differentiating with respect to the spatial coordinate yields
\begin{equation*}
\begin{split}
\alpha_x(t,x) & = u_x(t,x) + \gamma_\alpha'(x) X(t) \\
& + K_{uu}(x,x) u(t,x) + \int_0^x (K_{uu})_x(x,y) u(t,y) dy \\
& + K_{uv}(x,x) v(t,x) + \int_0^x (K_{uv})_x(x,y) v(t,y) dy 
\end{split}
\end{equation*}
Therefore, in order for $\alpha$ to verify the target PDE \eqref{eq:first_target_system}, the functions $K_{uu}$ and $K_{uv}$ and $\gamma_\alpha$ must verify the following \textit{kernel equations}:
\begin{equation}\label{eq:kernel_equations_alpha}
\left\{
\begin{array}{l}
     \lambda  K_{uv}(x,x) + K_{uv}(x,x) \mu + \eta^{+-}(x) = 0 \\
     \lambda (K_{uu})_x(x,y) + (K_{uu})_y(x,y) \lambda + K_{uv}(x,y) \eta^{-+}(y) = 0 \\
     \lambda (K_{uv})_x(x,y) - (K_{uv})_y(x,y) \mu + K_{uu}(x,y) \eta^{+-}(y) = 0 \\
     K_{uu}(x,0) \lambda Q - K_{uv}(x,0) \mu + \gamma_\alpha(x) B = 0 \\
     \lambda \gamma_\alpha'(x) + \gamma_\alpha(x) A + K_{uu}(x,0) \lambda M  = 0 \\
     \gamma_\alpha(0) = -M
\end{array} 
\right.
\end{equation}
Similarly, in order for $\beta$ to verify the target PDE \eqref{eq:first_target_system}, the functions $K_{vu}$ and $K_{vv}$ and $\gamma_\beta$ must verify the following \textit{kernel equations}:
\begin{equation}\label{eq:kernel_equations_beta}
\left\{
\begin{array}{l}
     - \mu  K_{vu}(x,x) - K_{vu}(x,x) \lambda + \eta^{-+}(x) = 0 \\
     - \mu (K_{vu})_x(x,y) + (K_{vu})_y(x,y) \lambda + K_{vv}(x,y) \eta^{-+}(y) = 0 \\
     - \mu (K_{vv})_x(x,y) - (K_{vv})_y(x,y) \mu + K_{vu}(x,y) \eta^{+-}(y) = 0 \\
     K_{uu}(x,0) \lambda Q - K_{uv}(x,0) \mu + \gamma_\beta(x) B = 0 \\
     - \mu \gamma_\beta'(x) + \gamma_\beta(x) A  + K_{vu}(x,0) \lambda M = 0 \\
     \gamma_\beta(0) = K
\end{array} 
\right.
\end{equation}

We find in the literature the following result on the well-posedness of these kernel equations \cite{auriol_minimum_2016}.
\begin{theorem}
    The kernel equations \eqref{eq:kernel_equations_alpha} and \eqref{eq:kernel_equations_beta} are well-posed and yield a unique solution $(K_{uu}, K_{uv}, K_{vu}, K_{vv}, \gamma_\alpha, \gamma_\beta)$.
\end{theorem}
The backstepping transformation is therefore well defined. Since both systems are equivalent because of the invertibility of the transform, we now only consider the target system.
\textcolor{blue}{More comments?}

In order to control the input of the target PDE \eqref{eq:first_target_system} with an effective adapted signal $V_{eff}$, we set the following feedback law for $V_{in}$:
\begin{equation}\label{eq:feedback_law_Vin_to_Veff_PDE_target}
\begin{split}
    V_{in}(t) & = V_{eff}(t) - R u(t,1) - \gamma_\beta(1) X(t) \\
    & - \int_0^1 K_{vu}(x,y) u(t,y) dy - \int_0^1 K_{vv}(x,y) v(t,y) dy.
\end{split}
\end{equation}
Mind that suppressing the term $R u(t,1)$ causes our control operator to become improper. This can cause some robustness issues, notably, the feedback loop can become unstable if exposed to some unaccounted delay \cite{auriol_delay-robust_2018}. Some methods have been developed to mitigate the instabilities, such as low-pass filters. We will not go into more details as it is out of the scope of this study. 
%In numeric simulations, we have to compute the kernels and the functions $\gamma$ in order to apply this feedback law. We discuss this in more details later.
\textcolor{blue}{More comments?}





\subsection{Trajectory tracking}
The explicit solution of $\beta$ shows that in order to control the SDE of the original sytem \eqref{eq:coupled_PDE_SDE}, we can focus on controlling the input-delayed stochastic differential equation with random coefficients
\begin{equation}\label{eq:equivalent_delayed_SDE}
\left\{
\begin{array}{l}
     dX(t) = (A X(t) + B U(t-h) + r(t)) dt + \sigma(t) dW_t  \\
     X(0) = X_0
\end{array} 
\right.
\end{equation}
where we denote $h \triangleq \frac{1}{\mu}$ and 
$$
r(t) \triangleq B \int_{t-\delta}^t \gamma_\beta \left( \mu (t-s) \right) \sigma(s) dW_s.
$$
Indeed, if we find a control $U$ that minimizes the covariance in the delayed SDE \eqref{eq:equivalent_delayed_SDE}. We can produce a control that minimizes the covariance of the original system \eqref{eq:coupled_PDE_SDE} by setting $V_{eff} = U$ and compute the associated controlled $V_{in}$. 
From now on, we therefore only focus on controlling the delayed SDE.

\textcolor{orange}{Mettre cette partie avant la WP (cf notes)}

\subsection{Artstein transformation of the SDE}
\textcolor{blue}{See next section}








\textcolor{orange}{--------------------------------------------------------------------------------------------------------------------------------------------------}



\subsection{Well-posedness of the closed loop}

We now show the well-posedness of the target system and some regularity properties of the solution. 

\textcolor{orange}{We now verify the well posedness of the target system with a control that verifies some properties}

We achieve these results by first solving the target system \eqref{eq:first_target_system} explicitly through the characteristic method. This method yields the following expression for $\beta$ :
\begin{equation}\label{eq:explicit_formula_beta}
\beta(t,x) = V_{eff}\left(t - \frac{1-x}{\mu} \right) + \int_{t-\frac{1-x}{\mu}}^t \gamma_\beta \left( x + \mu (t-s) \right) \sigma(s) dW_s.
\end{equation}
This process is  adapted to $\mathcal{F}_t$ for all $x \in [0,1]$. Let us show now that the SPDE is well-posed :
\textcolor{orange}{is adapted as the integrand is adapted etc}
\begin{lemma}\label{lem:well_posed_SPDE_L2}
    If $V_{eff}$ is in $L^2_\mathcal{F}([0,T]; \mathbb{R})$, then $t \mapsto \beta(t,\cdot)$ is in $L^2_\mathcal{F}([0,T] ; L^2(0,1))$. Moreover, if $V_{eff}$ is in $C^2_\mathcal{F}([0,T]; \mathbb{R})$, then $t \mapsto \beta(t,\cdot)$ is in $C^2_\mathcal{F}([0,T] ; L^2(0,1))$.
\end{lemma}
\begin{proof}
%As for the well-posedness of the solution, since $\gamma_\beta$ is in $L^\infty(0,1)$, we obtain through a classical theorem of stochastic partial differential equations \cite{hairer_introduction_2009}[Theorem 6.10] that the stochastic convolution term 
Since $\gamma_\beta$ is in $L^\infty(0,1)$, we obtain through a classical theorem of stochastic partial differential equations \cite{hairer_introduction_2009}[Theorem 6.10] that the stochastic convolution term 
$$
t \mapsto \int_{t-\frac{1-\cdot}{\mu}}^t \gamma_\beta \left( \cdot + \mu (t-s) \right) \sigma(s) dW_s
$$
is sample path continuous in $L^2(0,1)$. 
Therefore, we have
\begin{align*}
\Vert \beta & \Vert_{L^2_\mathcal{F}([0,T] ; L^2(0,1))}  \leq \Vert V_{eff} \Vert_{L^2_\mathcal{F}} \\
& + \left \Vert \int_{\cdot-\frac{1-\cdot_x}{\mu}}^\cdot \gamma_\beta \left( \cdot_x + \mu (\cdot-s) \right) \sigma(s) dW_s \right \Vert_{C^2_\mathcal{F}([0,T] ; L^2(0,1))}
\end{align*}
as well as
\begin{align*}
\Vert \beta & \Vert_{C^2_\mathcal{F}([0,T] ; L^2(0,1))} \leq \Vert V_{eff} \Vert_{C^2_\mathcal{F}} \\
& + \left \Vert \int_{\cdot-\frac{1-\cdot_x}{\mu}}^\cdot \gamma_\beta \left( \cdot_x + \mu (\cdot-s) \right) \sigma(s) dW_s \right \Vert_{C^2_\mathcal{F}([0,T] ; L^2(0,1))}
\end{align*}
\end{proof}
Let us now study the regularity of $t \mapsto \beta(t,x)$ for a fixed $x \in [0,1]$. 
\begin{lemma}\label{lem:regularity_beta}
     Let $x$ be in $[0,1]$. If $V_{eff}$ is in $L^2_\mathcal{F}([0,T]; \mathbb{R})$, then $t \mapsto \beta(t,x)$ is in $L^2_\mathcal{F}([0,T] ; L^2(0,1))$. Moreover, if $V_{eff}$ is in $C^2_\mathcal{F}([0,T]; \mathbb{R})$, then $t \mapsto \beta(t,x)$ is in $C^2_\mathcal{F}([0,T] ; L^2(0,1))$.
\end{lemma}
\begin{proof}
We obtain from the Burkholder-Davis-Gundy inequality \cite{le_gall_brownian_2016} that, for any $x \in [0,1]$, the stochastic process
$$
t \mapsto \int_{t-\frac{1-x}{\mu}}^t \gamma_\beta \left( x + \mu (t-s) \right) \sigma(s) dW_s
$$
is is sample path continuous in $\mathbb{R}$. We conclude in the same way as in the previous lemma.
\end{proof}

\textcolor{orange}{\begin{itemize}
    \item Faire la meme pour la WP de alpha et X (faire un seul lemme)
    \item Parler de l'inversibilité et l'utiliser pour faire un corollaire qui établit la well posedness du systeme initial.
    \item 
\end{itemize}}

\textcolor{blue}{Some comments on how the two previous lemma are similar? I could be wrong, but I feel both are necessary since we cannot obtain one from the other in a straightforward way. Also : should I do one big lemma instead ?}









